The Progression of Disparities within the Criminal Justice System: Differential Enforcement and Risk Assessment Instruments

Algorithmic risk assessment instruments (RAIs) increasingly inform decision-making in criminal justice. RAIs largely rely on arrest records as a proxy for underlying crime. Problematically, the extent to which arrests reflect overall offending can vary with the person's characteristics. We examine how the disconnect between crime and arrest rates impacts RAIs and their evaluation. Our main contribution is a method for quantifying this bias via estimation of the amount of unobserved offenses associated with particular demographics. These unobserved offenses are then used to augment real-world arrest records to create part real, part synthetic crime records. Using this data, we estimate that four currently deployed RAIs assign 0.5--2.8 percentage points higher risk scores to Black individuals than to White individuals with a similar \emph{arrest} record, but the gap grows to 4.5--11.0 percentage points when we match on the semi-synthetic \emph{crime} record. We conclude by discussing the potential risks around the use of RAIs, highlighting how they may exacerbate existing inequalities if the underlying disparities of the criminal justice system are not taken into account. In light of our findings, we provide recommendations to improve the development and evaluation of such tools.

==> Archive/Old/text/abstract.tex <==



 

==> Archive/Old/text/introduction.tex <==




==> Archive/Old/text/notation.tex <==

\section{Notation}
\label{sec:notation}

\begin{table}
\caption{Notation table}
\label{tab:notation}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{p{0.15\linewidth} p{0.1\linewidth} p{0.2\linewidth} p{0.55\linewidth}}
\multirow{6}{*}{Crime state}     & $C$                                     & Crime               &                                                                        \\
                                 & $I$                                     & Incident            & A crime that was recorded by the police                          \\
                                 & $I_R$                                   & Reported Incident   & An incident that was reported to the police  \\
                                 & $I_D$                                   & Discovered Incident & An incident that was discovered by the police                           \\
                                 & $A$                                     & Arrest              & An incident where an arrest has been made                               \\
                                 & $V$                                     & Conviction          & An incident that resulted in a conviction~                               \\ 
                                 & $J$                                     & Prison Sentence          & An incident that resulted in a prison or jail sentence                               \\ 
\cline{1-4}
\multirow{5}{*}{Crime attribute} & $K$                                     & Individual        &                                                                        \\
                                 & $S$                                     & Subgroup            & A subgroup of individuals                                           \\
                                 & $L$                                     & Location            & Location where the crime occurred, e.g., city or neighborhood                                       \\
                                 & $Y$                                     & Crime type        & The type of crime committed, e.g., assault, theft, etc.           \\
                                 & $T$                                     & Time                & Time when the crime was committed~                                     \\ 
\cline{1-4}
\multirow{2}{*}{Probabilities}  & \multicolumn{2}{l}{$P(I_D = 1\mid C=1, S=g_0, L=l_a) $} & \multirow{2}{*}{The probability that a 
crime becomes a discovered incident, }\\
 & \multicolumn{2}{l}{or $P^{g_0, l_a}_{C\rightarrow I_D}$ (short form)} & {given the subgroup the offender and the location of the crime} \\
\end{tabular}%
}
\end{table}

%Crimes, reported incidents, arrests, convictions
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Let $C\in\{0,1\}$ denote a random variable such that $C=1$ if a crime was committed by some individual in the population and $C=0$ otherwise. 
Similarly, let $I\in\{0,1\},$ $A\in\{0,1\},$ $V\in\{0,1\}$, $J\in\{0,1\}$ indicate whether the committed crime results in a \emph{recorded incident}, 
\emph{arrest}, \emph{conviction}, 
and a \emph{prison sentence} respectively.\footnote{We refer to all incarnation sentences, whether to be carried out in a jail or a prison as prison sentence.} 
We also refer to incidents as \emph{observed crimes}. 
The relationships between variables $C, I, A, V, J$ can be visualized in Figure \ref{fig:pipeline}.
We use the arguments $k,y,t,l$ to indicate that a crime of type $y$ (such as assault) was committed by individual $k$, on day $t$ at location $l$, e.g., $C(k,y,t,l)$. 
Analogous notation is adopted for the other random variables.
% Different pathways for recording incidents, and convictions. %Enforcement ratios
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
We make the simplifying assumption that an individual can be arrested only if they have committed a crime, i.e., $C=0$ implies $I=0$. 
Recorded incidents can be a product of reactive policing from reporting by victims or third parties,
or of proactive policing through other methods of discovery such as stop and search. 
We use $I_R=1$ to denote the former and $I_D=1$ to denote the latter.
% To estimate the probability that a recorded incident will lead to an arrest or a conviction, 
% we can look at the proportion of incidents that resulted in an arrest, and in a conviction, respectively. 
% However, since crimes committed are not observed, the probability that a crime will lead to a recorded incident cannot be directly calculated.
% Include explicit equations for these?
% Subgroups
Lastly, for an individual within the population, let $S$ denote membership of different subgroups. For example,  $S=0$ can indicate white individuals and $S=1$ black individuals. 
To simplify the presentation of the results, we will use $P^{s}_{C\rightarrow I}$ to refer to $P(I=1 \mid C=1, S=s)$, and similarly for other variables. We refer to $P^{s}_{C\rightarrow I}$ as an \emph{enforcement probability}. A summary of the notation used in this work is in Table~\ref{tab:notation}.

==> Bias in the CJ pipeline (4)/Archive/Old/text/abstract.tex <==



 

==> Bias in the CJ pipeline (4)/Archive/Old/text/introduction.tex <==




==> Bias in the CJ pipeline (4)/Archive/Old/text/notation.tex <==

\section{Notation}
\label{sec:notation}

\begin{table}
\caption{Notation table}
\label{tab:notation}
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{p{0.15\linewidth} p{0.1\linewidth} p{0.2\linewidth} p{0.55\linewidth}}
\multirow{6}{*}{Crime state}     & $C$                                     & Crime               &                                                                        \\
                                 & $I$                                     & Incident            & A crime that was recorded by the police                          \\
                                 & $I_R$                                   & Reported Incident   & An incident that was reported to the police  \\
                                 & $I_D$                                   & Discovered Incident & An incident that was discovered by the police                           \\
                                 & $A$                                     & Arrest              & An incident where an arrest has been made                               \\
                                 & $V$                                     & Conviction          & An incident that resulted in a conviction~                               \\ 
                                 & $J$                                     & Prison Sentence          & An incident that resulted in a prison or jail sentence                               \\ 
\cline{1-4}
\multirow{5}{*}{Crime attribute} & $K$                                     & Individual        &                                                                        \\
                                 & $S$                                     & Subgroup            & A subgroup of individuals                                           \\
                                 & $L$                                     & Location            & Location where the crime occurred, e.g., city or neighborhood                                       \\
                                 & $Y$                                     & Crime type        & The type of crime committed, e.g., assault, theft, etc.           \\
                                 & $T$                                     & Time                & Time when the crime was committed~                                     \\ 
\cline{1-4}
\multirow{2}{*}{Probabilities}  & \multicolumn{2}{l}{$P(I_D = 1\mid C=1, S=g_0, L=l_a) $} & \multirow{2}{*}{The probability that a 
crime becomes a discovered incident, }\\
 & \multicolumn{2}{l}{or $P^{g_0, l_a}_{C\rightarrow I_D}$ (short form)} & {given the subgroup the offender and the location of the crime} \\
\end{tabular}%
}
\end{table}

%Crimes, reported incidents, arrests, convictions
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Let $C\in\{0,1\}$ denote a random variable such that $C=1$ if a crime was committed by some individual in the population and $C=0$ otherwise. 
Similarly, let $I\in\{0,1\},$ $A\in\{0,1\},$ $V\in\{0,1\}$, $J\in\{0,1\}$ indicate whether the committed crime results in a \emph{recorded incident}, 
\emph{arrest}, \emph{conviction}, 
and a \emph{prison sentence} respectively.\footnote{We refer to all incarnation sentences, whether to be carried out in a jail or a prison as prison sentence.} 
We also refer to incidents as \emph{observed crimes}. 
The relationships between variables $C, I, A, V, J$ can be visualized in Figure \ref{fig:pipeline}.
We use the arguments $k,y,t,l$ to indicate that a crime of type $y$ (such as assault) was committed by individual $k$, on day $t$ at location $l$, e.g., $C(k,y,t,l)$. 
Analogous notation is adopted for the other random variables.
% Different pathways for recording incidents, and convictions. %Enforcement ratios
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
We make the simplifying assumption that an individual can be arrested only if they have committed a crime, i.e., $C=0$ implies $I=0$. 
Recorded incidents can be a product of reactive policing from reporting by victims or third parties,
or of proactive policing through other methods of discovery such as stop and search. 
We use $I_R=1$ to denote the former and $I_D=1$ to denote the latter.
% To estimate the probability that a recorded incident will lead to an arrest or a conviction, 
% we can look at the proportion of incidents that resulted in an arrest, and in a conviction, respectively. 
% However, since crimes committed are not observed, the probability that a crime will lead to a recorded incident cannot be directly calculated.
% Include explicit equations for these?
% Subgroups
Lastly, for an individual within the population, let $S$ denote membership of different subgroups. For example,  $S=0$ can indicate white individuals and $S=1$ black individuals. 
To simplify the presentation of the results, we will use $P^{s}_{C\rightarrow I}$ to refer to $P(I=1 \mid C=1, S=s)$, and similarly for other variables. We refer to $P^{s}_{C\rightarrow I}$ as an \emph{enforcement probability}. A summary of the notation used in this work is in Table~\ref{tab:notation}.
